Model Selection with Model Zoo via Graph Learning

Pre-trained deep learning (DL) models are increasingly accessible in public repositories, i.e., model zoos. Given a new prediction task, finding the best model to fine-tune can be computationally intensive and costly, especially when the number of pre-trained models is large. Selecting the right pre-trained models is crucial, yet complicated by the diversity of models from various model families (like ResNet, Vit, Swin) and the hidden relationships between models and datasets. Existing methods, which utilize basic information from models and datasets to compute scores indicating model performance on target datasets, overlook the intrinsic relationships, limiting their effectiveness in model selection. In this study, we introduce TransferGraph, a novel framework that reformulates model selection as a graph learning problem. TransferGraph constructs a graph using extensive metadata extracted from models and datasets, while capturing their inherent relationships. Through comprehensive experiments across 16 real datasets, both images and texts, we demonstrate TransferGraph's effectiveness in capturing essential model-dataset relationships, yielding up to a 32% improvement in correlation between predicted performance and the actual fine-tuning results compared to the state-of-the-art methods.

==> sections/algorithm.tex <==
\begin{algorithm}[t]
\caption{Select model candidates for finetuning on target dataset}
\label{algo:graph-selection}
\begin{algorithmic}[1]
\Require $M$: model set, $\chi$: dataset collection (including target dataset), $\phi$: dataset similarity, $T$: training history, $S$: predicted scores, $metadata$ \rihan{give metadata a notation?, where is it used below?}
\State $graph$ $\gets$ Construct a graph with \{$M$, $\chi$, $\phi$, $T$, $S$\}
% \State $graph$ $\gets$ Split the graph and get trainset
% \State $gnn$ $\gets$ Implement a graph learner and initiate it
\State $g\_learner$ $\gets$ train a graph learner with $graph$
% \State $emb\_dataset$ $\gets$ Get embeddings of the target dataset node with the trained $gnn$
\State $emb\_model$ $\gets$ \{\}
\For{$m \in M$}
\State $emd$ $\gets$ $g\_learner$ Get embeddings of the target model node with the trained $gnn$
\State add $emd$ to $emb\_model$
\EndFor
\State $distance$ $\gets$ Compute pairwise distance between $emb\_dataset$ and $emb\_model$
\State candidates $\gets$ Top $k$ models with the closest $distance$ values to the target dataset node $d_T$
\State \Return candidates
\end{algorithmic}
\end{algorithm}

==> sections/result_table.tex <==
\renewcommand{\arraystretch}{1.1}

\begin{table}[tb]
    \centering
    \begin{tabular}{p{1.6cm}|p{3.5cm}|c}
        \hline
       {\textbf{Methods}}  &  {\textbf{(Meta) Features}} & \textbf{Average Correlation} \\
       \hline\hline%[.1em]
        LogME & -  & 0.368 \\
        % & NCE  &  & 0.096 \\
        \hline
       \multirow{3}{1.3cm}{LR} &  Basic & 0.262 \\
                               % & Node2Vec+ (TG) &  0.261 \\
                                &  Node2Vec+ (TG), Basic &  0.337 \\
                    %  & & Basic, $d$ & 0.134 \\\cline{3-3}
                    % & Basic, $d$ & 0.314 \\
                                % & Node2Vec+ (TG), $d$ & \textbf{0.633} \\
                    & Node2Vec+ (TG), Basic, $d$  & \textbf{0.505} \\\cline{3-3}
       \hline
       % \hline
       \multirow{3}{2cm}{RF} & Basic & 0.579 \\
                             % &  Node2Vec+ (TG) & 0.593 \\
                             &  Node2Vec+ (TG), Basic &  0.583 \\
        % & & Basic, $d$ & 0.134 \\\cline{3-3}
        % & Basic, $d$ & 0.614 \\
                            % & Node2Vec+ (TG), $d$ & \textbf{0.633} \\
                            & Node2Vec+ (TG), Basic, $d$ & \textbf{0.633} \\
       \hline
       \multirow{3}{*}{XGBoost} &  Basic & 0.529 \\
                            % & & Basic, $d$ &  0.647 \\\cline{2-3}
                            % & Node2Vec+ (TG)  & 0.564 \\
                            & Node2Vec+ (TG), Basic & 0.57    \\
                            % & Node2Vec+ (TG), $d$ & 0.495 \\
                            & Node2Vec+ (TG), Basic, $d$  & \textbf{0.645}\\
                               % & \multirow{3}{2.2cm}{TG-GraphSAGE (Ours)} & - &  0.611 \\\cline{3-3}
                               % &  & Basic &  0.627 \\%\cline{3-3}
                               % & & Basic, $d$ & 0.575 \\\cline{3-3}
       \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:avg_corr}
\end{table}
\renewcommand{\arraystretch}{1}

% \begin{table}[tb]
%     \centering
%     \begin{tabular}{p{1.6cm}|p{2.3cm}|p{2.cm}|p{1.43cm}}
%         \hline
%        {\textbf{Methods}}  & {\textbf{Graph Features}} & {\textbf{(Meta) Features}} & \textbf{Average Correlation} \\
%        \hline\hline%[.1em]
%         LogME & -  & -  & 0.384 \\
%         % & NCE  &  & 0.096 \\
%         \hline
%        \multirow{5}{1.3cm}{LR} & - & Basic & 0.311 \\\cline{3-3}
%                     %  & & Basic, $d$ & 0.134 \\\cline{3-3}
%                     & & Basic, $d$ & 0.314 \\\cline{2-3}
        
%                     % & \multirow{3}{2.3cm}{TG-Node2Vec (Ours)}  & - & 0.256 \\\cline{3-3}
%                     %                             &  &  Basic &  0.3  \\%\cline{2-3}
%                     %                             & & Basic, $d$ &  \textbf{0.49}\\\cline{2-3}
%                     % & \multirow{3}{2.3cm}{TG-GraphSAGE (Ours)}  & - & 0.652 \\\cline{3-3}
%                     %                             &  &  Basic &  0.341 \\%\cline{2-3}
%                     %                             & & Basic, $d$ &  0.423\\\cline{2-3}
%                     & \multirow{3}{2.3cm}{TG-Node2Vec+ (Ours)} & - &  0.311 \\\cline{3-3}
%                                                 &  & Basic &  0.321 \\%\cline{3-3}
%                                                 & & Basic, $d$  & \textbf{0.487} \\\cline{3-3}
%        \hline
%        % \hline
%        \multirow{5}{2cm}{RF} & - & Basic & 0.584 \\\cline{3-3}
%         % & & Basic, $d$ & 0.134 \\\cline{3-3}
%         & & Basic, $d$ & 0.614 \\\cline{2-3}
%        % \hline
%        % \multirow{4}{*}{TG (Ours)} & \multirow{1}{*}{GraphSAGE} & \multirow{4}{2.3cm}{LogME, dataset distance, fine-tune accuracy}  & 0.475\\
%        %  & \multirow{1}{*}{GAT} &  & 0.502\\
%        %  & \multirow{1}{*}{GraphSAGE\_transfer} & & \textbf{}\\
%        %  & \multirow{1}{*}{GAT\_transfer} & & 0.508\\
%        % \hline
%        & \multirow{3}{2.2cm}{TG-Node2Vec (Ours)}  & - & 0.597 \\\cline{3-3}
%                                                            &  &  Basic &  0.582 \\
%                                                            & & Basic, $d$ & \textbf{0.632} \\\cline{2-3}
%                             % & \multirow{3}{2.2cm}{TG-GraphSAGE (Ours)} & - & 0.611 \\\cline{3-3}
%                             %                                &  & Basic &  0.595 \\%\cline{3-3}
%                             %                                & & Basic, $d$  & 0.624 \\\cline{3-3}
%        \hline
%        \multirow{5}{*}{XGBoost} & - & Basic & 0.551 \\\cline{3-3}
%                             % & & Basic, $d$ & 0.134 \\%\cline{3-3}
%                             & & Basic, $d$ &  0.647 \\\cline{2-3}
%                             % & \multirow{3}{2.2cm}{TG-Node2Vec (Ours)}  & - & 0.611 \\\cline{3-3}
%                             %                                &  &  Basic &    0.57 \\%\cline{2-3}
%                             %                               & & Basic, $d$  & \textbf{0.670}\\\cline{2-3}
%                             & \multirow{3}{2.2cm}{TG-Node2Vec+ (Ours)}  & - & 0.594 \\\cline{3-3}
%                                                            &  &  Basic & 0.568    \\%\cline{2-3}
%                                                           & & Basic, $d$  & \textbf{0.666}\\\cline{2-3}
%                                % & \multirow{3}{2.2cm}{TG-GraphSAGE (Ours)} & - &  0.611 \\\cline{3-3}
%                                % &  & Basic &  0.627 \\%\cline{3-3}
%                                % & & Basic, $d$ & 0.575 \\\cline{3-3}
%        \hline
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:avg_corr}
% \end{table}
% \renewcommand{\arraystretch}{1}


% \renewcommand{\arraystretch}{1.2}
% \begin{table*}[htb]
%     \centering
%     \begin{tabular}{p{1.6cm}|c|c|c|c|c|c|c|c|c}
%         \hline
%        \multirow{2}{*}{\textbf{Metric}} & \multirow{2}{*}{\textbf{Method}}&  \multicolumn{8}{c}{\textbf{Datasets}} \\\cline{3-10}
%          & & \textbf{kitti} & \textbf{cifar100} & \textbf{svhn} & \textbf{caltech101} & \textbf{pets} &  \textbf{dtd} & \textbf{stanfordcars} & \textbf{flowers}\\\hline\hline
%         \multirow{3}{*}{Correlation} & LogME & 0.654 & \textbf{0.614} & \textbf{0.237} & 0.487 & 0.349 & 0.324 & 0.438 & 0.246 \\
%                                     & NCE & 0.349 & -0.089 & 0.181 & 0.039 & -0.026 & -0.143 & 0.256 & -0.123\\
%                                     % & XGB & 0.505 & 0.108 & -0.027 & 0.805 & 0.806 & \textbf{0.895} & 0.621 & \textbf{0.82} \\
%                                     & TG-XGB\{N2V,basic\} & \textbf{0.745} & 0.33 & 0.120 & \textbf{0.83} & \textbf{0.825} & \textbf{0.885} & \textbf{0.825} & \textbf{0.795}\\\hline
%                                     % & TG-XGB\{N2V+,basic\} & 0.592 & 0.177 & 0.306 & 0.868 & 0.794 & 0.838 & 0.759 & 0.691 \\
%         \multirow{3}{*}{APK@20} & LogME & 0.356 & 0.555 & \textbf{0.478} & 0.688 & 0.269 & 0.378 & 0.638 & 0.530\\
%                                 & NCE & 0.066 & \textbf{0.563} & 0.450 & \textbf{0.736} & 0.319 & 0.287 & 0.554 & 0.349\\
%                                 % & XGB & 0.294 & 0.278 & 0.229 & 0.565 & \textbf{0.365} & 0.281 & 0.550 & 0.444\\
%                                 & TG-XGB\{N2V,basic\} & \textbf{0.462} & 0.270 & 0.357 & 0.675 & \textbf{0.351} & \textbf{0.528} & \textbf{0.871} & \textbf{0.562} \\\hline
%         \multirow{3}{1.8cm}{Avg. Accuracy (Top 20)} & LogME & 0.928 & \textbf{0.918} & \textbf{0.939} & 0.951 & \textbf{0.942} & 0.704 & 0.633 & 0.960 \\
%                                         & NCE & 0.919 & 0.917 & 0.939 & 0.954 & 0.939 & 0.668 & 0.642 & 0.848\\
%                                         % & XGB & \textbf{0.934} & 0.901  & 0.925 & 0.952 & 0.938 & 0.706 & 0.637 & 0.957 \\
%                                         & TG-XGB\{N2V,basic\} & \textbf{0.933} & 0.902 & 0.927 & \textbf{0.958} & 0.936 & \textbf{0.722} & \textbf{0.678} & \textbf{0.966} \\
%        \hline
%        % \multicolumn{2}{c|}{\textbf{Std. of the model performance on the datasets}} & 0.023 & 0.035 & 0.058 & 0.066 & 0.082 & 0.087 & 0.107 & 0.135 \\\hline
% \end{tabular}
%     \caption{Performance of different model selection strategy. We compare them on three different metrics, i.e., Pearson Correlation, APK@20, the avg accuracy of the top 20 returned models.}
%     \label{tab:avg_corr}
% \end{table*}
